Active Inference of Extended Finite State Machine Models with Registers and Guards

Extended finite state machines (EFSMs) model stateful systems with internal data variables and have numerous applications in software engineering. A major advantage of this type of model lies in its ability to model both the data flow and the data-dependent control behaviour. In the absence of such models, it is desirable to reverse-engineer them by observing the system's behaviour. However, existing approaches generally require the ability to reset the system during inference, or can only handle situations where the control flow depends exclusively on the input parameters, and not on the values of the stored data. In this work, we present a black-box active learning algorithm that infers EFSMs with guards and registers, and which significantly relaxes the assumptions that have to be made about the system in comparison to previous attempts.

==> sections/annex_algos.tex <==
%\newpage
%\vspace{1cm}
\SetStartEndCondition{ }{}{}%
% \SetKwProg{Fn}{Function}{\string}{}
\SetKwFunction{Range}{range}%%
\SetKw{KwTo}{in}\SetKwFor{For}{for}{\string:}{}%
\SetKwIF{If}{ElseIf}{Else}{if}{ then}{elif}{else}{}%
\SetKwFor{While}{while}{:}{fintq}%
\SetKwRepeat{Repeat}{\addtocounter{AlgoLine}{-1}repeat}{\nl until}%
\SetKwFor{For}{for}{ do}{}%
\SetKw{Return}{return}%

% \SetKwComment{Comment}{\color{blue}$\triangleright$\it}{\color{black}}%

% \newcommand{\Comm}[1]{%
% \color{blue} $\triangleright\,${\textit{#1}}\color{black}}%


% \renewcommand{\forcond}{$i$ \KwTo\Range{$n$}}
\AlgoDontDisplayBlockMarkers\SetAlgoNoEnd%\SetAlgoNoLine%
\DontPrintSemicolon

\SetKwFunction{Backbone}{\textrm{\textsc{Backbone}}}
\SetKwFunction{Home}{\textrm{\textsc{Home}}}
\SetKwProg{Fn}{Function}{}{}
\SetKw{Init}{Initializing:}

\setcounter{AlgoLine}{0}

\begin{algorithm}
%    \begin{algorithmic}[1]
\nl        \Fn(\Comment{Apply h until we can know the state reached}){\Home{$T,r,h$}}{
\nl        \Repeat{$q \neq \bot$} {% \label{home:repeat}
\nl             $(T,a,r) \gets \textsc{Apply}(T,r,h)$ \label{home:apply-homing}%
           \Comment{Apply $h$, observe response $a$, update regs}
\\
\nl
           let $\eta=\pi(a) \in O^*$
            \Comment{State reached is associated to $\eta$}\\
% The following If statement may be omitted if we accept "undefined for some w" in a loose sense meaning empty set
% That condition on H(\eta) undefined was more like a program than an algo
% to avoid null pointers. Any H(eta) is supposed to be empty set when
% referred to in the right end side of the \gets
%            \If{$H(\eta)$ is undefined} \label{backbone:reached-first-time}
%                \State $H(\eta) \gets \emptyset$
%            \EndIf
\nl            \If(\Comment{Learn characterization of tail state}){$H(\eta)$ is undefined for some $w \in W$}{  \label{home:partially-learnt}
\nl                $(T,y,r) \gets \textsc{Apply}(T,r,w)$\\
\nl                $H(\eta) \gets H(\eta) \cup \{w \mapsto \pi(y)\}$ \label{home:add-w}
%                \State continue - go to line \ref{home:repeat}
%                \Comment{Continue with next loop iteration}
}
\nl            \Else(\Comment{We know the state reached after $h/a$}){
\nl                let $q = (H(\eta),\rho_w(r,\epsilon))$ be the state reached at end of $h$
%  \Comment{$\rho_w(r,\sigma)$ first applies register updates from i/o sequence $\sigma$ to $r$, then projects on $R_w$}\\
\nl                $Q \gets Q \cup \{q\}$; $A(\pi(a))(q,r) \gets \epsilon$
  \Comment{$A$ records known access to configuration $(q,r)$ from homing tail}
}%            \EndIf
}%         \Until {$q \neq \bot$}
\nl         \Return $(T,q,r)$
~ \\
~ \\
}%        \EndFunction
%    \end{algorithmic}
    \caption{Homing into a known state}
    \label{func:home}
\end{algorithm} % home


\setcounter{AlgoLine}{0}

\begin{algorithm}[ht!]
    % \LinesNumbered
    % \SetAlgoLined
    \nl \Fn{\Backbone{$T,I_1,I_s,h,W,Q,\Delta,\Lambda$}}{
    \nl    \Init{$H \gets \emptyset$, $J \gets I_1$,
                 $q \gets \bot$, $r \gets \bot$} \\
%    \nl    \Repeat{$\Delta,\Lambda$ are complete over $I_s$ on a Scc}{
    \nl    \Repeat{no further sampling reachable in current Scc}{
    \nl       \If(\Comment{We do not know where we are}){$q = \bot$}{
    \nl          $(T,q,r) \gets \textsc{Home}(T,r,h)$
              }
    \nl       $(q',r',X,Y,r_1) \gets
                 \textsc{Transfer}(q,r,\Delta,\Lambda,I_1,J\setminus I_1)$
              \Comment{Target next transition to learn/sample} \\
    \nl       \If{such a path cannot be found}{
    \nl           goto line \ref{backbone:Scc}
                 \Comment{Graph not connected, try connecting with $I_s$}
              }
    \nl       \If(\Comment{$\pi(X)$ is not enabled in $q',r'$}){%
                 $Y = \Omega$ of $\omega$}{
    \nl          $\Lambda(q',\pi(X),\omega) \gets \{r',X,Y,r_1\}$,
                 $\Delta(q',\pi(X),Y) \gets q'$
                 \label{backbone:Omega} \\
    \nl          $q \gets q'$, $r \gets r'$
                 \Comment{We continue learning from the same state}
              }
    \nl       \Else(\Comment{$ {(q',r')} - X/Y \to \mathbf{(q'',r_1)} \to
                  w/\xi \to (q''',r_2)$}){%
    \nl           Let $q'' = \Delta(q',\pi(X),\pi(Y))$
                  \Comment{$q''$ (and so $\Delta$) might be a
                     ``state under construction''} \\
    \nl           \If(\Comment{We are sampling new values of a known transition
                            with same abstract output}){%
                      $q''$ is fully defined}{%
                            %and \exists X',Y'$ s.t.
                            % $\pi(Y)=\pi(Y')$ and $\pi_2(\Lambda(q',X'))=Y'$}
    \nl               $\Lambda(q',\pi(X),\pi(Y)) \gets
                      \Lambda(q',\pi(X),\pi(Y)) \cup \{(r',X,Y,r_1)\}$,
                      \Comment{No different $Y'$ with
                            same $r'$ unless (W-)inconsistency} \\
    \nl               $q \gets \Delta(q',\pi(X),\pi(Y))$, $r \gets r_1$
                  }
    \nl           \Else(\Comment{Learn tail of transition from $q'$
                              on input $X$}){%
    \nl               for some $w \not\in dom (\pi_1(q''))$,
                      \label{backbone:learn-trans} \\
    \nl                  \qquad $(T,\xi,r_2) \gets \textsc{Apply}(T,r_1,w)$
                         \label{backbone:add-to-dictionary} \\
    \nl               $\Lambda(q',\pi(X),\pi(Y)) \gets
                      \Lambda(q',\pi(X),\pi(Y)) \cup \{(r',X,Y,r_1)\}$ \\
    \nl               $\pi_1(q'')(w)) \gets \pi(\xi)$
                         \label{backbone:update-delta}
                         \Comment{Update $\Delta$,$\pi_1$ is 1st element of couple} \\
    \nl               \If{$dom(\pi_1(q''))=W$}{%
    \nl                  $Q \gets Q \cup \{(\pi_1(q''),\rho_w(r_1,\epsilon)\}$\\
    \nl                  $A \gets \textsc{UpdateAccess}(T, q'',
                                                        \rho_w(r_1,\epsilon))$
                         \Comment{We record shortest access
                                  to $(q'',r_1)$ from $(q,r)$ or
                                  last homing in $T$} \\
% Note that Delta(q',X.w) could be undefined so q would also get \bot
    \nl                  $q \gets \Delta^*(q',\pi(X.w),\pi(Y.\xi))$
                         {if defined else}
                         $q \gets \bot $ \\
    \nl                  $r \gets r_2$}
    \nl              \Else{%
    \nl                  $q \gets \bot $}
                  }

% In the following line, Delta is defined when the tail state is known
% for each input/output pair that appears in Delta
% WARNING: don't we need Lambda to compute Scc with concrete values ?
    \nl
                  \If(\Comment{$\Delta^-$ trims the $\Delta$ graph from $h/a$ by cutting transitions that cannot be accessed with $A$ and $\Lambda$}){$\Delta^-(\Delta,\Lambda,h,a,A)$
                     (where $h/a$ was latest homing in $T$) is defined and
                      contains a complete strongly connected component (Scc)}{%
    \nl              $J \gets I_s$
                     \label{backbone:Scc}
                  }
              }
         }
    \nl \Return{$T, Q, \Delta, \Lambda$}
        \label{backbone:Exit}
    }
~ \\
~ \\
    \caption{Backbone procedure with guards on registers}
    \label{alg:backbone}
\end{algorithm}


\setcounter{AlgoLine}{0}

\SetKwFunction{Transfer}{\textrm{\textsc{Transfer}}}

\begin{algorithm}
    \nl \Fn(\Comment{We look for deterministic transfer, either through
                     unguarded transitions, or when registers and input
                     determine known transitions}){%
            \Transfer{$q, r, \Delta, \Lambda, I_1, I_2$}}{%
    \nl     \Comment{To reach a given input configuration $r'$, we record
                     the list of parameter values that can be set by unguarded
                     transitions while building the path, and can adapt the
                     parameter values at the end to set values to $r'$} \\
    \nl     \Comment{First we look for a short transfer with a bounded search
                     ($k \geq 0$ is the bound, tailorable), and if that fails,
                     we resort to a path from re-homing}
% For easier implementation, we could just start implementing with k=0.
% Actually alpha is a bit special because it contains concrete inputs but only abstract outputs. We are not fully consistent here?
            \label{transfer:shortest-alpha} \\
    \nl     Find short(-est) $\alpha \in (\mathcal{I} \times O)^k$ and
            $X \in I_1$ with $\Delta^*(q,\pi(\alpha))=q'$ and \\
            $\rho_w(r,\alpha)=\pi_2(q')=\rho_w(r',\epsilon)$
            s.t. $\pi_1(\Delta(q',\pi(X),*))$ is partial,
            \Comment{First try to learn new input from a state, in its
                     reference configuration} \\
    \nl     \Comment{``partial'' means either not defined at all, or
                     there is an output whose characterisation is partial;
                     if $\Omega$ was the output for $\pi(X)$ it is not
                     partial regardless of $r'$ and $X$; if it was
                     $\omega$ for a given $r'$ and $X$, we can still look
                     for a different $r'$ or $X$.} \\
    \nl     or $\exists r' \neq \pi_2(q'), Y \neq Y'$
            s.t. $\rho_g(r,\alpha)=\rho_g(r',\epsilon)$ and \\
            $\{(\pi_2(q'),X,Y,*),(r',X,Y',*)\} \subset
            \Lambda(q',\pi(X),\pi(Y))$ and \\
            $\pi_1(\Delta(q',\pi(X),\pi(Y')))$ is partial
            \Comment{or a guarded transition} \\
    \nl     \If(\Comment{(otherwise) no transition to learn in current Scc}){%
                previous fails}{%
    \nl         Find $\alpha$ and $X \in I_2$ s.t.
                $\Lambda(q',\pi(X),*)$ does not contain $(*,X,*,*)$
                \Comment{transfer to a transition to be sampled} \\
    \nl         $q'=\Delta^*(q,\pi(\alpha))$, $r'=\rho(r,\alpha)$
            }
    \nl     \If(\Comment{bounded search failed, resort to homing}){%
                all previous fail}{%
    \nl         $(T,a,r) \gets \textsc{Apply}(T,r,h)$ and
                update $\Lambda$ on the way (if transitions are in $Q$) \\
    \nl         \If{$\Delta^-(\Delta,\Lambda,h,\pi(a),A)$ no longer contains
                    unsampled states and transitions}{%
    \nl             \Return{no path found}
                    \Comment{all transitions in reachable Scc already sampled
                             on $I_2$, transfer fails}
                }
    \nl         Look by BFS for shortest sequence
                $\alpha$ in $\Delta^-(\Delta,\Lambda,h,\pi(a),A)$,
                pick $A(\pi(a))(q',r')=\alpha$ and $X$ s.t.
                $\pi_1(\Delta(q',\pi(X),*))$ is partial or has guarded
                transition to partial state, or failing that has a transition
                to be sampled
            }
            \Comment{Here $q', r', \alpha, X$ are defined. If $\Delta$ was
                     partial in $q$, then $\alpha=\epsilon$, $q'=q$} \\
% We are in q,r; alpha will lead us to q',r' where we need to learn transition on X
% and by X/Y we will go to q'',r1.
% We overload Apply to accept not just input sequences, but IO sequences
% Now we attempt transferring
    \nl     $(T,\beta,r') \gets \textsc{Apply}(T,r,\alpha)$ and
            update $\Lambda$ on the way \\
%             \Comment{State is now $q'$ unless some abstract output differed}
    \nl     \If(\Comment{Transfer stopped prematurely on differing output}){%
                $\beta \neq \pi_o(\alpha)$}{%
    \nl         let $\beta=\beta'.o'$,
                $\alpha=\alpha'.X.\alpha''/\beta'.o.\beta''$
                s.t. $\pi_o(\alpha')=\beta', o' \neq o$ \\
    \nl         $Y \gets o'$, $r_1 \gets r', r' \gets
                   \rho(r,\alpha'), q' \gets \Delta^*(q,\alpha')$
% IMPORTANT note: thanks to observability and W being assumed correct, we know the LAST transition was guarded
% If W was not correct, then it could be a W-ND and could come from an earlier transition
                \Comment{We found a new guarded transition} \\
    \nl         \Comment{If h or W were not correct, we should handle
                         inconsistency if after $\alpha'$ we have same input
                         configuration $r$ for $o$ and $o'$}
            }
    \nl     \Else(\Comment{$(q,r) - \alpha(')/\beta(') \to
               \mathbf{(q',r')} - X/Y \to (q'',r_1) \to w/\xi \to (q''',r_2)$}){%
    \nl          $(T,Y,r_1) \gets \textsc{Apply}(T,r',X)$
            }
    \nl     $A \gets \textsc{UpdateAccess}(T,q',r')$
            \Comment{We record the shortest access to $(q',r')$ from $(q,r)$
                     or the last homing in $T$} \\
    \nl     \Return $(q',r',X,Y,r_1)$
        }
~ \\
~ \\
    \caption{Transferring from $q, r$ to next transition to learn}
    \label{func:transfer}
\end{algorithm}

\setcounter{AlgoLine}{0}

% \SetKwFunction{ehW}{\textrm{\textsc{ehW}}}

\begin{algorithm}
    \SetAlgoLined
    \nl \KwIn{$I_1 \subset I_2 \subset I_s \subset \mathcal{I}$,
            $W \subset I_1^*$, $R_w \subset R_g \subset R$}
    \nl     $h \in I_1^+$, s.t. $\rho_g(\bot,h)$ has a value
            for each register in $R_g$ \\
    \nl     \Init{$T \gets \epsilon$} \Comment{$T$ is the learning trace}\\
    \nl     \label{falg:repeat}
            \Repeat{no counterexample found}{%
    \nl         $Q, \Delta, \Lambda \gets \emptyset$, $I_o \gets I_1$ \\
    \nl         \Repeat{\textsc{Backbone} terminates with
                        no inconsistency}{%
    \nl             $T,Q,\Delta,\Lambda \gets$
                    \textsc{Backbone}($T,I_1,I_o,h,W,Q,\Delta,\Lambda$) \\
                % With assumption h and W are correct, no update needed below
    \nl         handle inconsistencies on the way to update $h,W,I_1$
%                \Comment{if h \& W not trustable} \\
% The for loop could be "hidden" inside the GetNFSMCounterExample function
    \nl         \For{$I_o$ incrementally ranging from $I_1$
                     to $I_1 \cup R_w(I_2)$}{%
    \nl              \Comment{Sampling on $R_w(I_2)$ first to have
                              smallest set of register configs
                              to compare, hence smallest number of redundant
                              states}

    \nl             $T,Q,\Delta,\Lambda \gets$
                    \textsc{Backbone} ($T,I_1,I_o,h,W,Q,\Delta,\Lambda$)
                }
    \nl         $I_o \gets I_1 \cup R_g(I_2)$ \\
    \nl         $T,Q,\Delta,\Lambda \gets$
                \textsc{Backbone} ($T,I_1,I_o,h,W,Q,\Delta,\Lambda$) \\
% RG: I am not sure that at this point we need to incremental search and starting from Rw(I2)
% RG Maybe we could directly do it for I2.
    \nl         \For{$I_o$ incrementally ranging from $I_1$
                     to $I_1 \cup R_w(I_2)$ then ${} \cup R_g(I_2)$}{%
    \nl              $(T,\mathit{CE}) \gets
                     \textsc{GetNFSMCounterExample}
                        (T,Q,\Delta,\Lambda,\mathit{SUL},I_o)$
                     \Comment{Ask for a CE using only inputs from $I_o$}  \\
    \nl              \If{CE found}{%
    \nl                  $(W,I_1,I_s,Q,\Delta,\Lambda) \gets$
                         \textsc{ProcessCounterexample}
                         \Comment{If W changed, this resets $Q,\Delta,\Lambda$}\\
                         \Comment{At this point, $I_s$ would not be changed} \\
    \nl                  continue to start of repeat \textsc{Backbone} loop
                     }
                }
    \nl         $I_o \gets I_s$
                \Comment{If $R_g$ is correct, $I_s$ will not change NFSM,
                         just feed \textsc{generalise}}
            }
% Still wondering whether we should reduce after each backbone or just before generalizing.
% It makes sense to try finding CE on a smaller structure, but as there is no unique reduction, could this trigger instability ?
% At the same time, sampling on a non-reduced NFSM provides more diverse samples, even
% if some are redundant once reduced. So we do it just for helping \textsc{generalise}.
% For sure, following our experiment with Michael's tool, it is definitely useful to
% reduce before calling \textsc{generalise}.
    \nl     $(Q,\Delta,\Lambda) \gets
            \textsc{reduceFSM} (Q,\Delta,\Lambda)$
            \Comment{Reduce, not Minimize, as there is no unique minimum} \\
    \nl     \Repeat{$\neg$ (CE is a data CE)}{%
    \nl         $M \gets$
                \textsc{generalise}($T,h,Q,I,O,P_I,P_O,\Delta,\Lambda$) \\
    \nl         $(T,\mathit{CE}) \gets
                \textsc{GetCounterExample}(M,\mathit{SUL})$
            }
    \nl     \If{CE found}{%
    \nl         $(W,I_1,I_s,Q,\Delta,\Lambda) \gets$
                \textsc{ProcessCounterexample}
                \Comment{If W modified, $Q,\Delta,\Lambda$ are reset}
            }
        }
    \nl \Return{$M$}
~ \\
~ \\
    \caption{Main ehW algorithm}
    \label{alg:full-algo}
\end{algorithm}

